Mathematical models for nonlinear ultrasound contrast imaging with microbubbles

Ultrasound contrast imaging is a specialized imaging technique that applies microbubble contrast agents to traditional medical sonography, providing real-time visualization of blood flow and vessels. Gas-filled microbubbles are injected into the body, where they undergo compression and rarefaction and interact nonlinearly with the ultrasound waves. Therefore, the propagation of sound through a bubbly liquid is a strongly nonlinear problem that can be modeled by a nonlinear acoustic wave equation for the propagation of the pressure waves coupled via the source terms to a nonlinear ordinary differential equation of Rayleigh-Plesset type for the bubble dynamics. In this work, we first derive a hierarchy of such coupled models based on constitutive laws. We then focus on the coupling of Westervelt's acoustic equation to Rayleigh-Plesset type equations, where we rigorously show the existence of solutions locally in time under suitable conditions on the initial pressure-microbubble data and final time. Thirdly, we devise and discuss numerical experiments on both single-bubble dynamics and the interaction of microbubbles with ultrasound waves.

==> abk.tex <==
\nomenclature{$p$}{pressure of the liquid \nomunit{[\si{\pascal}]}}\label{key}
\nomenclature{$\rho_l$}{mass density of the liquid \nomunit{[\si[per-mode=symbol]{\kilogram\per\cubic\meter}]}}
\nomenclature{$\rho_g$}{mass density of the gas \nomunit{[\si[per-mode=symbol]{\kilogram\per\cubic\meter}]}}
\nomenclature{$\rho$}{mass density of the mixture \nomunit{[\si[per-mode=symbol]{\kilogram\per\cubic\meter}]}}
%\nomenclature{$\bmass = \bmass_0 + \bmass'$}{volume concentration}
\nomenclature{$\bfu$}{liquid and gas velocity \nomunit{[\si[per-mode=symbol]{\meter\per\second}]}}
\nomenclature{$n$}{bubble number density \nomunit{[\si[per-mode=symbol]{1\per\cubic\meter}]}}
\nomenclature{$R$}{bubble radius \nomunit{[\si{\meter}]}}
\nomenclature{$v$}{volume \nomunit{[\si{\cubic\meter}]}}
\nomenclature{$\mu$}{shear viscosity \nomunit{[\si{\pascal \second}]}}
\nomenclature{$\mu_b$}{bulk viscosity \nomunit{[\si{\pascal \second}]}}
%\nomenclature{$c_l$}{liquid sound speed}
\nomenclature{$\frac{B}{A}$}{nonlinearity parameter \nomunit{[1]}}
\nomenclature{$\kappa$}{adiabatic exponent for microbubbles \nomunit{[1]}}
%\nomenclature{$\kappa_0$}{adiabatic factor for microbubbles \nomunit{[1]}}
\nomenclature{$c_v$}{heat capacity at constant volume \nomunit{[\si[per-mode=symbol]{\joule\per\kelvin}]}}
\nomenclature{$c_p$}{heat capacity at constant pressure \nomunit{[\si[per-mode=symbol]{\joule\per\kelvin}]}}
\nomenclature{$\tau$}{relaxation time parameter \nomunit{[\si{\second}]}}
\nomenclature{$\alpha$}{order of the fractional derivative \nomunit{[1]}}
\nomenclature{$\beta$}{nonlinearity coefficient \nomunit{[1]}}
%\nomenclature{$s$}{specific entropy \nomunit{[\si[per-mode=symbol]{\joule\per\kilogram\per\kelvin}]}}
%\nomenclature{$T$}{absolute temperature \nomunit{[\si{\kelvin}]}}
%\nomenclature{$\tau_{\text{th}}$}{relaxation time characteristic of the medium \nomunit{[\si{\second}]}}
\nomenclature{$p_{\text{int}}$}{internal pressure \nomunit{[\si{\pascal}]}}
\nomenclature{$p_{\text{ext}}$}{external pressure \nomunit{[\si{\pascal}]}}
%\nomenclature{$\mu_l$}{liquid viscosity \nomunit{[\si{\pascal \second}]}}
\nomenclature{$\pv$}{vapor pressure \nomunit{[\si{\pascal}]}}
\nomenclature{$p_{\text{stat}}$}{static ambient pressure \nomunit{[\si{\pascal}]}}
\nomenclature{$\sigma$}{surface tension at the liquid-gas interface of the bubble \nomunit{[\si[per-mode=symbol]{\newton\per\meter}]}}
\nomenclature{$\gamma$}{adiabatic index in the tissue \nomunit{[1]}}
\nomenclature{$p_{\text{pgn}}$}{gas pressure inside the bubble at rest \nomunit{[\si{\pascal}]}}
\nomenclature{$R_0$}{radius at equilibrium \nomunit{[\si{\meter}]}}
\nomenclature{$c$}{speed of sound \nomunit{[\si[per-mode=symbol]{\meter\per\second}]}}
\nomenclature{$\chi$}{shell elasticity \nomunit{[\si[per-mode=symbol]{\newton\per\meter}]}}
\nomenclature{$\sigma_0$}{surface tension of the bubble at rest \nomunit{[\si[per-mode=symbol]{\newton\per\meter}]}}
\nomenclature{$\kappa_s$}{shell viscosity \nomunit{[\si[per-mode=symbol]{\kilogram\per\second}]}}
%\nomenclature{$k(x)$}{nonlinearity coefficient}
%\nomenclature{$\delta$}{viscous damping coefficient \nomunit{[\si[per-mode=symbol]{\newton\second\per\meter}]}}
%\nomenclature{$\omega_0, \, \eta, \, a, b$}{constants in alternative representation for ODE in terms of $v$}
\nomenclature{$\eta$}{coupling constant \nomunit{[\si[per-mode=symbol]{\kilogram\per\meter^6}]}}
\nomenclature{$b$}{sound diffusivity \nomunit{[\si[per-mode=symbol]{\square\meter\per\second}]}}
%\nomenclature{$t$}{time coordinate}
%\nomenclature{$x$}{space coordinate}
%\nomenclature{$\delta_p$}{pressure data size}
%\nomenclature{$\delta_R$}{bubble data size}
%\nomenclature{$\tilde{T}$}{final time}
%\nomenclature{$\Omega$}{domain}
%\nomenclature{$(R_0, R_1)$}{initial radius data}
%\nomenclature{$(p_0, p_1)$}{initial pressure data}
%\nomenclature{$\lambda$}{adaptive time index}
\nomenclature{$A$}{amplitude of the driving pressure \nomunit{[\si{\pascal}]}}
\nomenclature{$f$}{frequency of the driving pressure \nomunit{[\si{\hertz}]}}
\nomenclature{$\bmass$}{gas volume fraction \nomunit{[1]}}
